Heterogeneous Bitwidth Binarization in Convolutional Neural Networks

Recent work has shown that fast, compact low-bitwidth neural networks can be surprisingly accurate. These networks use homogeneous binarization: all parameters in each layer or (more commonly) the whole model have the same low bitwidth (e.g., 2 bits). However, modern hardware allows efficient designs where each arithmetic instruction can have a custom bitwidth, motivating heterogeneous binarization, where every parameter in the network may have a different bitwidth. In this paper, we show that it is feasible and useful to select bitwidths at the parameter granularity during training. For instance a heterogeneously quantized version of modern networks such as AlexNet and MobileNet, with the right mix of 1-, 2- and 3-bit parameters that average to just 1.4 bits can equal the accuracy of homogeneous 2-bit versions of these networks. Further, we provide analyses to show that the heterogeneously binarized systems yield FPGA- and ASIC-based implementations that are correspondingly more efficient in both circuit area and energy efficiency than their homogeneous counterparts.

==> algorithms/middle_out.tex <==
\begin{algorithm}[!ht]
  \caption{Middle-out bit selection and binary approximation calculation.}
  \textbf{Input:} A tensor $T$ with batches or filters and a mapping $B$ between bitwidths and the fraction of $T$ to binarize to that bitwidth. \\
  \textbf{Output:} A heterogeneous binary approximated tensor $T^B$ and a mapping $M^B$ indicating the number of bits used for each value of $T^B$. 
  \begin{algorithmic}[1]
  	\State $M^B = 0$
    \For{$k^{th}$ batch of $T$} \Comment{binarization performed independently for each batch or filter}
    	\State $P_k = \text{sort}(|(|T_k| - \text{mean}(|T_k|)|)$ \Comment{Sort indices by proximity to mean (middle-out selection)}
    	\For{(bitwidth, fraction) in $B$} \Comment{iterate through low-first sorted bitwidths}
    		\State $I$ = $P_k$.Pop($\text{fraction} \times T_k$.Size) \Comment{Pop the values closest to the mean to binarize}
    		\For{$i$ in $I$}
	    		\State $M^B_{ki} = $ bitwidth
	    	\EndFor
    	\EndFor
    	\State $T^B_k = 0$ \Comment{bit map $M^B_k$ calculated, now compute approximation}
		\For{$i$ from $1$ to max bitwidth} \Comment{constructively calculate the values of all bitwidths}
			\For{$M^B_{kj} \geq i$} \Comment{only calculate bits above $i$}
				\State $T^B_{kj} \pluseq$ mean($|T_{kj}|$) $\times$ sign($T_{kj}$) \Comment{mean($|T_{kj}|$) is the scalar for bit $i$, sign($T_{kj}$)}
				\State $T_kj \minuseq$ mean($|T_{kj}|$) $\times$ sign($T_{kj}$) \Comment{update residual error}
			\EndFor
		\EndFor
    \EndFor
  \end{algorithmic}
  \label{middleout}
\end{algorithm}


==> figures/binw_acc.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.7]{figures/binw_acc_vs_bits.png}
\end{center}
\caption{Accuracy of HBNN AlexNet of varying bitwidth between 1 and 2 bits compared to state of the art binarization and the full precision network.}
\label{binw_acc}
\end{figure}

==> figures/cifar10.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.7]{figures/cifar10.png}
\end{center}
\caption{HBNN accuracy trained on CIFAR-10 with uninformed layer-level bit distribution.}
\label{cifar10}
\end{figure}


==> figures/representational_power.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.8]{figures/EuclidRep.png}
\end{center}
\caption{Ability of different binarization schemes to approximate a large tensor of normally distributed random values. A bit composition denoted as x/y/z indicates x\% of values are binarized to 1-bit, y\% to 2-bit, and z\% to 3-bit.}
\label{representational_power}
\end{figure}


==> figures/testfig.tex <==
\begin{figure*}
\centering
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/cifar10.png}
\caption{Fully connected layers}
\label{fig:vgg16-fc}
\end{subfigure}
~
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/cifar10.png}
\caption{Latency of convolution op "conv2-1"}
\end{subfigure}
~
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/cifar10.png}
\caption{Latency of convolution op "conv4-2"}
\end{subfigure}
~
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/cifar10.png}
\caption{Workspace memory of ``conv2-1''}
\end{subfigure}
~
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/cifar10.png}
\caption{Workspace memory of ``conv4-2''}
\end{subfigure}
~
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/cifar10.png}
\caption{End-to-end latency of VGG16}
\label{fig:model-lat}
\end{subfigure}
\caption{Latency per input in the batch for (a) fully-connected, (b) pooling operation, and (c) activation operation.}
\label{fig:batch}
\end{figure*}
